Using newest VLT-KMOS HII Galaxies and other cosmic tracers to test the $\Lambda$CDM tension

We place novel constraints on the cosmokinetic parameters by using a joint analysis of the newest VLT-KMOS HII galaxies (HIIG) with the Supernovae Type Ia (SNIa) Pantheon sample. We combine the latter datasets in order to reconstruct, in a model-independent way, the Hubble diagram to as high redshifts as possible. Using a Gaussian process we derive the basic cosmokinetic parameters and compare them with those of $\Lambda$CDM. In the case of SNIa, we find that the extracted values of the cosmokinetic parameters are in agreement with the predictions of $\Lambda$CDM model. Combining SNIa with high redshift tracers of the Hubble relation, namely HIIG data, we obtain consistent results with those based on $\Lambda$CDM as far as the present values of the cosmokinetic parameters are concerned, but find significant deviations in the evolution of the cosmokinetic parameters with respect to the expectations of the concordance $\Lambda$CDM model.

==> pack.tex <==
\usepackage{times,graphics}
\usepackage[colorlinks]{hyperref}
\usepackage{makecell}
\usepackage{diagbox}

%showpacs
\usepackage{graphicx}
\usepackage{dcolumn}
\usepackage{bm}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{epstopdf}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{lipsum}
\usepackage{amssymb}
\usepackage{color}
\usepackage{dcolumn}
\usepackage{bm}
\usepackage{natbib}
\usepackage{tabu}
\usepackage{times,graphics}
\usepackage{makecell}
\usepackage{diagbox}

\RequirePackage{mathptmx}      % use Times fonts if available on your TeX system
\RequirePackage{flushend}
%\RequirePackage[numbers,sort&compress]{natbib}
%\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}




